Time Complexity of Broadcast and Consensus for Randomized Oblivious Message Adversaries

Broadcast and consensus are most fundamental tasks in distributed computing. These tasks are particularly challenging in dynamic networks where communication across the network links may be unreliable, e.g., due to mobility or failures. Indeed, over the last years, researchers have derived several impossibility results and high time complexity lower bounds (i.e., linear in the number of nodes $n$) for these tasks, even for oblivious message adversaries where communication networks are rooted trees. However, such deterministic adversarial models may be overly conservative, as many processes in real-world settings are stochastic in nature rather than worst case. This paper initiates the study of broadcast and consensus on stochastic dynamic networks, introducing a randomized oblivious message adversary. Our model is reminiscent of the SI model in epidemics, however, revolving around trees (which renders the analysis harder due to the apparent lack of independence). In particular, we show that if information dissemination occurs along random rooted trees, broadcast and consensus complete fast with high probability, namely in logarithmic time. Our analysis proves the independence of a key variable, which enables a formal understanding of the dissemination process. More formally, for a network with $n$ nodes, we first consider the completely random case where in each round the communication network is chosen uniformly at random among rooted trees. We then introduce the notion of randomized oblivious message adversary, where in each round, an adversary can choose $k$ edges to appear in the communication network, and then a rooted tree is chosen uniformly at random among the set of all rooted trees that include these edges. We show that broadcast completes in $O(k+\log n)$ rounds, and that this it is also the case for consensus as long as $k \le 0.1n$.

==> 9-conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

We studied the fundamental problems of broadcast and Consensus on dynamic networks from a randomized perspective, studying randomized oblivious message adversaries with parameter $k$. We showed that for small values of $k$ information dissemination is significantly faster compared to the deterministic setting.

We believe that our work opens several interesting avenues for future research. In particular, it would be interesting to extend our study of randomized oblivious message adversaries to other information dissemination problems and network topologies. We also believe that our techniques can be useful to analyze other dynamic models, including the SI model in epidemics.  




==> 96-rotatedtable.tex <==
\begin{landscape}
\section{Table of Results}

\begin{tabular}{|c |c |c |c|}
	\hline
	             & Broadcast                                                                                       & All-to-All Broadcast                                                                             & Consensus                                                                                       \\ \hline
	 Uniformly   &                                                                                                 &                                                                                                  &                                                                                                 \\
	   Random    & $O(c \cdot \log n), q \le n^{-c}$                                                               & $O(c \cdot \log n), q \le n^{1-c}$                                                               & $O(c \cdot \log n), q \le n^{-c}$                                                               \\
	Trees (URT)  & $\Omega(\log n)$                                                                                & $\Omega(\log n)$                                                                                 & $\Omega(\log n)$                                                                                \\ \hline
	  URT with   &                                                                                                 &                                                                                                  &                                                                                                 \\
	 Byzantine   & $O(c \cdot \log n), q \le n^{-c}$                                                               & $O(c \cdot \log n), q \le n^{1-c}$                                                               & $O(c \cdot \log n), q \le n^{-c}$                                                               \\
	   Nodes     & $\Omega(\log n)$                                                                                & $\Omega(\log n)$                                                                                 & $\Omega(f+\log n)$                                                                              \\ \hline
	  URT with   &                                                                                                 &                                                                                                  &                                                                                                 \\
	Adversarial  & $O(c \cdot (\log n+k)), q \le n^{-c}$                                                           & $O(c \cdot (\log n+k)), q \le n^{1-c}$                                                           & $O(c \cdot  (\log n+k)), q \le n^{-c}$                                                          \\
	   Edges     & $\Omega(\log n+k)$                                                                              & $\Omega(\log n + k)$                                                                             & $\Omega(\log n + k)$                                                                            \\ \hline
	  Directed   & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{-c}\log n$                               & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{1-c}\log n$                               & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{-c}\log n$                               \\
	Erdős–Rényi  & $O\left(\frac{c\log n}{\log (1+\frac m n)}\right), q \le n^{-c}\log n$ if $\frac m n \ge \ln n$ & $O\left(\frac{c\log n}{\log (1+\frac m n)}\right), q \le n^{1-c}\log n$ if $\frac m n \ge \ln n$ & $O\left(\frac{c\log n}{\log (1+\frac m n)}\right), q \le n^{-c}\log n$ if $\frac m n \ge \ln n$ \\
	Graphs (DER) & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                 & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                \\ \hline
	  DER with   &                                                                                                 &                                                                                                  &                                                                                                 \\
	 Byzantine   & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{-c}\log n$                               & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{1-c}\log n$                               & $O\left(\ceil{\frac{c}{m/n}} \log n\right)$, $q \le n^{-c}\log n$                               \\
	   Nodes     & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                 & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                \\ \hline
	  DER with   &                                                                                                 &                                                                                                  &                                                                                                 \\
	Adversarial  & $O\left(\ceil{\frac{c \cdot (n^2-m_a)}{(m-m_a)n}} \log n\right),    q \le n^{-c}\log n$         & $O\left(\ceil{\frac{c \cdot (n^2-m_a)}{(m-m_a)n}} \log n\right),    q \le n^{1-c}\log n$         & $O\left(\ceil{\frac{c \cdot (n^2-m_a)}{(m-m_a)n}} \log n\right),    q \le n^{-c}\log n$         \\
	   Edges     & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                 & $\Omega\left(\frac{\log n}{\log (1+m/n)}\right)$                                                \\ \hline
\end{tabular} 


\end{landscape}

==> consensuslowerbound.tex <==
\section{consensus lower bound}

\begin{theorem}\label{thm:lowerconsensus}
    Consensus in Uniformly random rooted trees fails to complete within $\frac {\log n} 2$ rounds with probability at least $\frac 1 2$.
\end{theorem}

To prove this result, we will first use the following theorem, which is due to F{\"{u}}gger, Nowak and Winkler~\cite{fugger2020radius}:

\begin{theorem}[Theorem 5 of~\cite{fugger2020radius}]
    Let $G$ be a dynamic network. Consider the $n$ parallel algorithms that try to achieve broadcast starting at the $n$ different nodes of $G$. Then no consensus algorithm terminates before at least one broadcast completes.
\end{theorem}

We will also use unimodal distributions:

\begin{definition}
    A probability distribution $(p_k)_{k \in [n]}$ on $[n]$ is unimodal if it has only one mode, that is, if there exists $\ell \in [n]$ such that for every $k < \ell$, $p_k \le p_{k+1}$, and $p_k \ge p_{k+1}$ otherwise.
\end{definition}

Keylon and Kester~\cite{keilson1978unimodality} have characterized the matrices that preserve unimodality:

\begin{theorem}
    A matrix $A$ preserves unmodality, that is $Ax$ is unimodal for every $x$ unimodal, iif $Q^{-1}AQ \in TP_2$, where $Q = (\1(i \ge j))_{1\le i,j\le n}$ is a lower triangular matrix, and $TP_2$ is the set of matrices whose all $2 \times 2$ minors have non-negative determinants.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:lowerconsensus}]
We know that if in a round $t$, the number of informed nodes is $N_t$, then in the next round, the probability distribution of $N_{t+1}-N_t$ is a binomial distribution of parameters $(n-N_t, \frac{N_t}{n})$. This is thus a Markov Chain, with transition matrix $A$, where $A_{ij} = {n-i \choose j-i} \left(\frac i n\right)^{j-i}\left(1-\frac i n\right)^{n-i}$. Note that $A_{ij} = 0 $ if $ i > j$. We will show that $A$ preserves unimodality.

Let us first compute $AQ$:

\begin{align*}
    (AQ)_{ik}&= \sum_{j \in [n]}A_{ij}Q_{jk}=\sum_{j \in [n]}A_{ij}\1(j \ge k) =\sum_{j = k}^n A_{ij} 
\end{align*}

And now $Q^{-1}AQ$:
    \begin{align*}
    (Q^{-1}AQ)_{\ell k}= \sum_{i \in [n]}Q^{-1}_{\ell i} (AQ)_{i k}&=(AQ)_{1k}= \sum_{j = k}^n A_{1j} & \text{if $\ell =1$}\\
    &= -(AQ)_{\ell -1,k} + (AQ)_{\ell, k} = -\sum_{j = k}^n A_{\ell-1,j} + \sum_{j = k}^n A_{\ell,j} &\text{otherwise}
\end{align*}

Let us now compute the determinant $d(\ell, k)$ of a minor, of indices $\ell$ and $k$, first if $\ell, k > 1$. Wlog, assume that $k > \ell$:

\begin{align*}
    d(\ell, k) &=  (Q^{-1}AQ)_{\ell \ell}(Q^{-1}AQ)_{k k} -(Q^{-1}AQ)_{\ell k}(Q^{-1}AQ)_{k \ell}\\
    &= \left( -\sum_{j = \ell}^n A_{\ell-1,j} + \sum_{j = \ell}^n A_{\ell,j}\right)
    \left( -\sum_{j = k}^n A_{k-1,j} + \sum_{j = k}^n A_{k,j}\right)\\& \quad\quad - 
    \left( -\sum_{j = k}^n A_{\ell-1,j} + \sum_{j = k}^n A_{\ell,j}\right)
    \left( -\sum_{j = \ell}^n A_{k-1,j} + \sum_{j = \ell}^n A_{k,j}\right)\\
    &= A_{\ell -1, \ell-1} \times A_{k-1, k-1} \ge 0
\end{align*}

If on the other hand $\ell = 1$:
\begin{align*}
    d(\ell, k) &=  (Q^{-1}AQ)_{\ell \ell}(Q^{-1}AQ)_{k k} -(Q^{-1}AQ)_{\ell k}(Q^{-1}AQ)_{k \ell}\\
    &= \sum_{j = 1}^n A_{1j}
    \left( -\sum_{j = k}^n A_{k-1,j} + \sum_{j = k}^n A_{k,j}\right)\\& \quad\quad - 
   \sum_{j = k}^n A_{1j}
    \left( -\sum_{j = \ell}^n A_{k-1,j} + \sum_{j = \ell}^n A_{k,j}\right)\\
    &=1 \times A_{k-1, k-1} \ge 0
\end{align*}








\end{proof}
